Unbounded orbits for the Plaid Model

This paper is a sequel to my paper "Introducing the Plaid Model". In this paper it is shown that the plaid model has unbounded polygonal paths for every irrational parameter. This result parallels my result that outer billiards on kites has unbounded orbits for every irrational parameter

==> 5rational.tex <==
\section{Even Rational Sequences}

\subsection{The Even Predecessor}

In this chapter we will develop the (very elementary)
number theory we need for the proof of the Copying Theorem.

Two rationals $p_1/q_1$ and $p_2/q_2$ are
{\it Farey related\/} if
\begin{equation}
p_1q_2 - p_2q_1 = \pm 1.
\end{equation}
In this case we write $p_1/q_1 \leftrightarrow p_2/q_2$.
We write $p_1/q_1 \leftarrow p_2/q_2$ if
$p_1+q_1<p_2+q_2$.   In this case, we call
$p_1/q_1$ a {\it predecessor\/} of $p_2/q_2$.
Each positive even rational $p_2/q_2$ in $(0,1)$
with $p_2>1$ has two predecessors, one of which
is even.  When $p_2/q_2=1/q_2$, we could take
the even predecessor to be $0/1$.

We call $p_2/q_2$ {\it major\/} if $2\omega_1<\omega_2$
and {\it minor\/} if $2\omega_1<\omega_2$.  Here
$\omega_k=p_k+q_k$ for $k=1,2$.  We never have equality
because $\omega_k$ is odd.


Here is how we find the even predecessor of $p_2/q_2$.
Let $t_2 \in (0,\omega_2/2)$ be the relevant solution to
\begin{equation}
\label{tuneX}
2p_2t_2 \equiv \pm 1 \hskip 15 pt {\rm mod\/} \hskip 5 pt \omega_2.
\end{equation}
This means that
$$2p_2t_2 = k_2(p_2+q_2) \pm 1.$$
Rearranging this, we get
$$p_2(2t_2-k_2) - q_2(k_2) = \pm 1$$
We have $k_2<\min(p_2,2k_2)$.  Setting 
$$p_0=k_2, \hskip 20 pt q_0=2t_2-k_2,$$
we see that $p_0/q_0 \leftarrow p_2/q_2$.
But $p_0/q_0$ is reduced and both $p_0$ and $q_0$
have the same parity.  Hence $p_0/q_0$ is the
odd predecessor.  The even predecessor is
\begin{equation}
p_1/q_1=\frac{p_2-k_2}{q_2-2t+k_2}.
\end{equation}
Note that
\begin{equation}
\omega_1=\omega_2-2t_2.
\end{equation}
From this we conclude that $p_2/q_2$ is
major if and only if $t_2>\omega_2/4$.


\subsection{The Alternate Predecessor}

It turns out that we need to understand a
different way to simplify rationals. 
Let $p_2/q_2$ be an even rational.
Let $\omega_2=p_2+q_2$.  The
quantity $\omega_2-2t_2$ has an
interpretation, in terms of our
plaid model, as the distance between
the two horizontal (or vertical) lines
of capacity 2.  In this section
we concentrate on the case then $t_2>\omega_2/3$.
We know in already that $p_2/q_2$ is minor.
Hence, the rational
\begin{equation}
p_3/q_3=\frac{p_2-2p_1}{q_2-2q_1}
\end{equation}
is a positive rational in reduced terms.
We call $p_3/q_3$ the {\it alternate predecessor\/}
of $p_2/q_2$ and we write $p_3/q_3 \Leftarrow p_2/q_2$.
\newline
\newline
{\bf Remark:\/}
The cases $p_2/q_2=2/(2k+1)$, which lead to $p_3/q_3=0/1$,
do not arise because $t_2<\omega_2/3$ in these cases.
\newline

We define $t_3$ relative to $p_3/q_3$ as in Equation
\ref{tuneX}.  

\begin{lemma}
$\omega_2-2t_2=\omega_3-2t_3$.
\end{lemma}

\startproof
We have
$$w_3=\omega_2-4t_2.$$
We define $u_3=3t_2-w_2$.  Note that
$\omega_2-2t_2=\omega_3-2u_3$.
So, to finish the proof, we just have
to check that $u_3=t_3$.  By hypothesis,
we have $u_3>0$.  Since 
$0<\omega_2-2t_2=\omega_3-2u_3$, we have
$u_3 \in (0,\omega_3/2)$.  So, we just have
to check that $2p_3u_3 \equiv \pm 1$ mod $\omega_3$.
We will consider the case when $2p_2t_2 \equiv 1$ mod $\omega_2$.
The other case works the same way.

In the case at hand, we have
$$k_2=\frac{2p_2t_2-1}{\omega_2}.$$
Using this equation, we compute
$$N:=\frac{2p_3u_3-1}{\omega_3}=
\frac{-3-2p_2^2-2p_2q_2 + 6p_2t_2}{\omega_2}.$$
Plugging in the equation
$6p_2t_2=3+3k_2\omega_2$ and factoring, we
see that $N$ is an integer.  Hence
$2p_3u_3 \equiv 1$ mod $\omega_3$.
\endproof

\begin{lemma}
Suppose that $p_3/q_3 \Leftarrow p_2/q_2$.
Then $p_3/q_3$ and $p_2/q_2$ have the
same even predecessor.
\end{lemma}

\startproof
Let $p_1/q_1 \leftarrow p_2/q_2$ be the even
predecessor of $p_2/q_2$.  We want to prove
that $p_1/q_1 \leftarrow p_3/q_3$ as well.
Once again, we have
$$
p_3/q_3=\frac{p_2-2p_1}{q_2-2q_1}
$$
We have $$\omega_3-\omega_1=
(\omega_2-2\omega_1)-(\omega_2-2t_2)=
2(t_2-\omega_1)=2(3t_2-\omega_2)>0.$$
Hence $\omega_1<\omega_3$.
A direct calculation shows that
$p_1/q_1$ and $p_3/q_3$ are
Farey-related.
Hence $p_1/q_1 \leftarrow p_3/q_3$.
\endproof

Now we change our notation somewhat,
in order to better do an interative
construction.
We call the rational $p/q$ a
{\it core parameter\/} if
$t(p/q)>\omega/3$.  Then we
have the alternate predecessor
$p'/q' \Leftarrow p/q$.  If
$p'/q'$ is a core parameter,
we may repeat the construction and produce
a longer chain of alternate predecessors
$p''/q'' \Leftarrow p'/q' \Leftarrow p/q$.
All these rationals have the same
even predecessor.  Continuing in
this way, we produce a maximal finite chain
\begin{equation}
p^{(n)}/q^{(n)} \Leftarrow \cdots \Leftarrow p/q.
\end{equation}
We call $p^{(n)}/q^{(n)}$ the
{\it core predecessor\/} of $p/q$.
We write
\begin{equation}
p^{(n)}/q^{(n)} \Longleftarrow p/q.
\end{equation}
The core predecessor of $p/q$ is not
a core parameter, but it has the same
even precessor as $p/q$.








\end{document}


Here we classify the even rationals in $(0,1)$
into $3$ types:
\begin{enumerate}
\item $p/q$ has {\it type 1\/} if
$\tau(p/q)<\omega/3$ and $p/q$ is major.
\item $p/q$ has {\it type 2\/} if
$\tau(p/q)<\omega/3$ and $p/q$ is minor.
\item $p/q$ has {\it type 3\/} if
$\tau(p/q)> 1/3$.
\end{enumerate}
We ignore $p/q=1/2$ in this classification.

Referring to the construction in \S \ref{mb},
the distance from the nearest line of capacity $2$
to the $y$-axis is $\tau_2=\tau(p/q)$, 
and the distance $\tau_4$ from
the nearest line of capacity $4$ to the $y$-axis
is $\tau_4=\min(\tau_2,\omega-\tau_2)$.
We have $\tau_4<\tau_2$ if and only if $p/q$ has
type $3$.

Now we prove some elementary lemmas about
this classification.

\begin{lemma}
Suppose that $p/q$ has type 3.   Then the
even predecessor $p/q$ is major.
\end{lemma}




\subsection{The Canonical Sequence}








\end{document}

==> Backup/4even.tex <==
\section{The Even Sequence}

\subsection{Even Predecessors}

This chapter contains some elementary
number theory which will be useful
in our proof.


Let $p'/q'$ and $p/q$ be two even rational
paramters.  We write
$p'/q' \leftarrow p/q$ if $|pq'-qp'|=1$ and
$\omega'<\omega$.  Here $\omega=p+q$ as usual.
We call $p'/q'$ the {\it even predecessor\/} of $p/q$.
This rational is unique.  

\begin{lemma}
\label{formula}
Suppose that $p'/q' \leftarrow p/q$.  Then
$2\omega'<\omega$ if and only if $\tau>\omega/4$.
\end{lemma}

\startproof
 There is some
integer $\theta$ so that
$$2p\tau = \theta(p+q) \pm 1.$$
Rearranging this, we get
$$p(2\tau-\theta) - q(\theta) = \pm 1$$
We have $\theta<\min(p,2\tau)$.  Setting 
$$p''=\theta, \hskip 20 pt q''=2\tau-\theta,$$
we see that $|p''q-q''p|=1$.
This implies that $p''/q''$ is in lowest
terms.  Moreover, both $p''$ and $q''$ are
odd.  That means that $p'=p-p''$ and $q'=q-q''$.
Hence
\begin{equation}
p'/q'=\frac{p-\theta}{q-2\tau+\theta}.
\end{equation}
Note that
\begin{equation}
\omega'=\omega-2\tau.
\end{equation}
The conclusion of this lemma is immediate
from the last equation.
\endproof

We write $\widehat p/\widehat q \Leftarrow p/q$ if
we have
\begin{equation}
\widehat p/\widehat q =p_0/q_0 \leftarrow  \cdots
\leftarrow p_n/q_n = p/q, \hskip 30 pt
2\omega_0<\omega_1.
\end{equation}
Here $\omega_k=p_k+q_k$.  




\subsection{The Even Sequence}

\begin{lemma}
\label{weak}
There exists a sequence
$\{p_n/q_n\}$ converging to
$A$ such that
$p_n/q_n \leftarrow p_{n+1}/q_{n+1}$
for all $n$.
\end{lemma}

\startproof
We have the usual Farey
triangulation of the hyperbolic plane $\H^2$ by
ideal triangles.  The geodesics
bounding these triangles join
rationals $p_1/q_1$ and $p_2/q_2$
such that $|p_1q_2-p_2q_1|=1$.
We call these geodesics the
{\it Farey Geodesics\/}.
Two of the Farey geodesics in the tiling
join the points $0/1$ and $1/1$ to $1/0$.
This last point is interpreted as the
point at infinity in the upper half
plane model of $\H^2$.  Let
$Y=\{(x,y)|\ 0<x<1\}$ be the
open portion of $\H^2$ between these
two vertical geodesics.

Each Farey geodesic in $Y$ which joins
two even rationals $p/q$ and $p'/q'$ 
can be oriented
so that it points from $p/q$ to $p'/q'$ if
and only if $p'/q' \leftarrow p/q$.
We leave the rest of the Farey geodesics
unoriented.

We claim that there is a backwards 
oriented path from
$0/1$ to $A$.  To see this, choose any
sequence of even rationals converging to $A$
and consider their sequence of even predecessors.
This gives us a sequence of finite directed
paths joining $0/1$ to rationals which
converge to $A$.  
Given the local finiteness
of the Farey triangulation -- meaning that
any compact subset of $\H^2$ intersects
only finitely many triangles -- we can
take a limit of these paths, at least on
a subsequence, and get a directed path
converging to $A$.  

Reading off the
vertices of this path gives us a
sequence $\{p_n/q_n\}$ with
$p_n/q_n \leftarrow p_{n+1}/q_{n+1}$
for all $n$.
\endproof

\begin{lemma}
\label{strong}
There exists a sequence
$\{p_n/q_n\}$ converging to
$A$ such that
$p_n/q_n \Leftarrow p_{n+1}/q_{n+1}$
for all $n$.
\end{lemma}

\startproof
Let $\{p_n/q_n\}$ be the 
sequence from Lemma \ref{weak}.
We just need
to prove that $2(p_n+q_n)<p_{n+1}+q_{n+1}$
infinite often.  If this is true, then some
subsequence of $\{p_n/q_n\}$ has the
desired properties for this lemma.

If this lemma is false, then we might
chop off the beginning and assume that
this never happens.  If $2(p_n+q_n)>p_{n+1}+q_{n+1}$
then we must have $r_{n-1}=2r_n-r_{n+1}$ for
$r \in \{p,q\}$.  Applying this iteratively,
we get that $r_{k}=(k+1)r_1-kr_0$ for $k=1,2,3,...$.
But then $\lim p_n/q_n=(p_1-p_0)/(q_1-q_0)$, which
is rational. This is a contradiction.
\endproof

\subsection{A Diophantine Estimate}

We call the sequence from Lemma \ref{strong}
the {\it even sequence\/} corresponding to $A$.

\begin{lemma}
Let $\{p_k/q_k\}$ be the even sequence corresponding
to $A$.  Then
$$|A-p_k/q_k|<4/\omega_k^2.$$
\end{lemma}

\startproof
For each fixed value of $k$, we have
some sequence
$$p_k/q_k \leftarrow p^*_k/q^*_k \leftarrow \cdots \leftarrow p_{k+1}/q_{k+1},$$
where $2\omega_k<\omega_k^*$.
We will consider the case when $p_k/q_k<p_k^*/q_k^*$.  
The other case has a similar treatment.
We introduce the new rational
$$p_k^{**}/q_k^{**}=\frac{p_k^*-p_k}{q_k^*-q_k}.$$
Note that the three rationals
$p_k/q_k$ and $p_k^*/q_k^*$ and
$p_k^{**}/q_k^{**}$ form the vertices of a
Farey triangle.  Moreover $p_k^*/q_k^*<p_k^{**}/q_k^{**}$
because $p_k^*/q_k^*$ is the Farey sum of
$p_k/q_k$ and $p_k^{**}/q_k^{**}$.

Given the geometry of the Farey graph, we have
$$A \in [p_k/q_k,p_k^{**}/q_k^{**}].$$
Moreover
$$|p_k/q_k-p_k^{**}/q_k^{**}|=\frac{1}{q_kq^{**}_k} \leq
\frac{1}{q_k^2}<\frac{4}{\omega_k^2}.$$
The second-to-last inequality comes from the
fact that $q_k^{**}>q_k$.
\endproof

\begin{corollary}
\label{dio1}
Let $P=2A/(1+A)$ and
$P_k=2p_k/(p_k+q_k)$.  Then we have 
$$|P-P_k|<8/\omega_k^2.$$
\end{corollary}

\startproof
Setting $A_k=p_k/q_k$, we have
$P_k=2A_k/(1+A_k)$.
The function $f(t)=2t/(1+t)$ is
$2$-lipschitz on the interval $[0,1]$.
Hence $$|f(A_k)-f(A)| \leq 2 |A_k-A| <8/\omega_k^2.$$
This completes the proof.
\endproof

\subsection{The Core Constant}
\label{kappa}

\noindent
{\bf Remark:\/}
The reader who is keen to see the broad outlines
of the proof of the Unbounded Orbits Theorem
might want to skip the remaining sections
of this chapter until later.  The material
in the rest of this chapter is not needed
until \S 6.
\newline

Define
\begin{equation}
F=\bigcup_{n=1}^{\infty} F_n, \hskip 30 pt
F_n=\frac{n}{2n+1}.
\end{equation}

Recall that $\omega=p+q$ and that
$\tau \in (0,\omega/2)$ has the property
that 
\begin{equation}
2\tau p \equiv \pm 1 \hskip 10 pt
{\rm mod\/} \hskip 5 pt \omega.
\end{equation}

\begin{lemma}
$\tau/\omega \in F$ if and only if
$p/q=1/2n$ for some $n$.
\end{lemma}

\startproof
Suppose that $\tau/\omega=n/(2n+1)$.
Then $2p\tau=p\omega-p=k\omega \pm 1$ for
some $k$.  This forces $p=1$.
At the same time, if $p/q=1/2n$, then
a direct calculation shows that
$\tau=n$ and hence $\tau/\omega=F_n$.
\endproof

\noindent
{\bf The Core Constant:\/}
Given the parameter $p/q$ we define
$\kappa=\kappa(p/q)$ to be the unique
integer such that
$\tau/\omega \in [F_{\kappa},F_{\kappa}+1)$.
We call $\kappa$ the {\it core constant\/}.
\newline

We want to interpret the core constant
in terms of the even predecessor. We
begin with a preliminary result.

\begin{lemma}
Suppose that $p'/q' \leftarrow p/q$.
Then $\tau \equiv \pm \tau'$ mod $\omega'$.
\end{lemma}

\startproof
We will assume that $2p\tau \equiv 1$ mod $\omega$.
The other case has a similar treatment.
We use the formulas from Lemma \ref{formula}.
We have 
$$2p\tau=\theta \omega +1=
\theta \omega'+2\tau \theta+ 1.$$
Rearranging, we get
$$\theta \omega ' + 1 =
2(p-\theta)\tau = 2p'\tau.$$
Hence $2p'\tau \equiv \pm 2p'\tau'$ mod $\omega'$.
Since $2p$ is relatively prime to $p+q$, we
get that $\tau \equiv \pm \tau'$ mod $\omega'$.
\endproof

Now we come to our alternate
interpretation of the core constant.

\begin{lemma}[Core]
\label{core00}
Suppose that $p'/q' \leftarrow p/q$.
Then $\tau \pm \tau'=\kappa \omega'$
for some choice of sign.
\end{lemma}

\startproof
For simplicity we consider
the case when $\tau \equiv \tau'$
mod $\omega'$. The other case has
a similar treatment. Note that we have $p>1$
because the rationals $1/2n$ do
not have even predecessors.

The quantity $t=\tau-\kappa \omega'$ satisfies
$2p't \equiv \pm 1$ mod $\omega'$.
So, we just have to show that
$t \in (0,\omega')$.
We compute
\begin{equation}
\tau-\kappa \omega'=\tau - \kappa(\omega-2\tau).
\end{equation}
After a bit of algebra, we see that
this expression lies in $(0,\omega')$ if and
only if
$$\tau/\omega \in (F_{\kappa},F_{\kappa+1}),$$
and this is true by definition.
\endproof

\newpage

==> Backup/5even.tex <==
\section{Some Elementary Number Theory}

\subsection{All About Predecessors}

We fix an even rational parameter
$p/q$.  To avoid trivialities, we assume
that $p>1$.  Given an even rational
parameter $p/q$, we make the
following definitions:
\begin{itemize}
\item $p'/q'$ is the even predecessor of $p/q$.
\item $\widehat p/\widehat q$ is the core
predecessor of $p/q$.
\item $p^*/q^*$ is the core predecessor of $p'/q'$.
\item $\omega=p+q$.
\item $\tau$ is the tune of $p/q$, as in \S \ref{tune}.
\item $\kappa$ is as in Lemma \ref{strong}.
\end{itemize}
We mean to define $\omega,\tau,\kappa$ for the
other parameters as well. Thus, for instance,
$\omega'=p'+q'$.


\begin{lemma}
\label{omnibus}
The following is true.
\begin{enumerate}
\item $\widehat p/\widehat q \in (0,1)$
is a rational in lowest terms.
\item Either
$\tau-\tau'=\kappa \omega'$ or
$\tau+\tau'=(1+\kappa) \omega'$.
In all cases, $\tau' \leq \tau$.
\item $p'/q'$ is also the even predecessor of
$\widehat p/\widehat q$.
\item $\widehat \kappa=0$.
\item $\omega-2\tau = \widehat \omega-2\widehat \tau$.
\item If $\kappa=0$ then $\tau'=\tau$ when
$\tau<\omega/4$ and $\tau'=\omega'-\tau$ when $\tau>\omega/4$.
\item If $\kappa \geq 1$ then $\kappa \widehat \omega<(3/2)\omega$.
\item If $\kappa' \geq 1$ then $\omega^*+\omega'<\omega$.
\end{enumerate}
\end{lemma}


\subsubsection{Statement 1}

We first give a formula for $p'/q'$.
 There is some
integer $\theta>0$ so that
$$2p\tau = \theta(p+q) \pm 1.$$
Rearranging this, we get
$$p(2\tau-\theta) - q(\theta) = \pm 1$$
We have $\theta<\min(p,2\tau)$.  Setting 
$$p''=\theta, \hskip 20 pt q''=2\tau-\theta,$$
we see that $|p''q-q''p|=1$.
This implies that $p''/q''$ is in lowest
terms.  Moreover, both $p''$ and $q''$ are
odd.  That means that $p'=p-p''$ and $q'=q-q''$.
Hence
\begin{equation}
\label{zoop}
\omega'=\omega-2\tau.
\end{equation}

We have
\begin{equation}
\label{gap}
\frac{\omega'}{\omega}=1-2\bigg(\frac{\tau}{\omega}\bigg)
\leq 1-2\bigg(\frac{\kappa}{2\kappa+1}\bigg)=\frac{1}{2\kappa+1}.
\end{equation}
If $2\kappa q' \geq q$ then Equation \ref{gap} implies
that $(2\kappa+1)p'+q' \leq p$. 
But then a short calculation shows 
that $|pq'-qp'|=p'q'>1$.
This is a contradiction.
Hence $2\kappa q'<q$.  The same
argument works with $p$ in place of $q$.

Since $\widehat p/\widehat q$ is Farey related
to $p'/q' \in (0,1)$, we see that $\widehat p/\widehat q$
also lies in $(0,1)$ and is in lowest terms.
This proves Statement 1.

\subsubsection{Statement 2}

We first prove that
$\tau \equiv \pm \tau'$ mod $\omega'$.
We will assume that $2p\tau \equiv 1$ mod $\omega$.
The other case has a similar treatment.  We
use the formulas that we have just derived.
We have 
$$2p\tau=\theta \omega +1=
\theta \omega'+2\tau \theta+ 1.$$
Rearranging, we get
$$\theta \omega ' + 1 =
2(p-\theta)\tau = 2p'\tau.$$
Hence $2p'\tau \equiv \pm 2p'\tau'$ mod $\omega'$.
Since $2p'$ is relatively prime to $\omega'$, we
get that $\tau \equiv \pm \tau'$ mod $\omega'$.

Suppose first that
$\tau \equiv \tau'$ mod $\omega'$.
The quantity $t=\tau-\kappa \omega'$ satisfies
$2p't \equiv \pm 1$ mod $\omega'$.
So, we just have to show that
$t \in (0,\omega')$.
We compute
\begin{equation}
t=\tau-\kappa \omega'=\tau - \kappa(\omega-2\tau)=
\tau(2\kappa+1)-\kappa\omega.
\end{equation}
After a bit of algebra, we see that
this expression lies in $(0,\omega')$.

When $\tau \equiv -\tau$ mod $\omega$, we
instead consider the quantity
$t=(\kappa+1)\omega-\tau$.  Again we
know that $2p't \equiv \pm 1$ mod $\omega'$.
The rest of the proof is very similar
to what is done in the other case.

Now we establish the second part of
Statement 1. We have one of the two equalities
$$\tau-\tau'=\kappa \omega', \hskip 30 pt
\tau+\tau'=(\kappa+1)\omega'.$$
In the first case, we obviously
have $\tau' \leq \tau$.  In
the second case, the same
inequality follows from
the fact that $\tau'<\omega'/2$.

\subsubsection{Statement 3}


Let $\widehat p/\widehat q$ be the core
predecessor of $p/q$.
Since
$\widehat p=p-2\kappa p'$ and $\widehat q=q-2\kappa q'$
the two rationals $p'/q'$ and $\widehat p/\widehat q$ are
both Farey related.
Equation \ref{gap}, which is a strict
inequality when $p>1$,  says that
$(2\kappa +1) \omega'< \omega$.
Since $\widehat \omega=\omega-2\kappa \omega'$,
we conclude that
$\omega'<\widehat \omega$.
Hence $p'/q'$ is the Farey predecessor
of $\widehat p/\widehat q$.
This completes the proof of Statement 3.

\subsubsection{Statement 4}

If Statement 4 is false, then
Equation \ref{gap}, applied to
$\widehat p/\widehat q$, tells us that
\begin{equation}
\widehat \omega-3\omega'>0.
\end{equation}
Combining this with the 
fact that 
$$\widehat \omega=\omega-2\kappa \omega'>0,$$
we can say that
$$\omega-(2\kappa+3)\omega'>0.$$
But then we have
$$
\frac{1}{2\kappa+3}=
1-2F_{\kappa+1}<
1-2\bigg(\frac{\tau}{\omega}\bigg)=
\frac{\omega'}{\omega}<
\frac{1}{2\kappa+3}.
$$
This is a contradiction.

\subsubsection{Statement 5}

The proof goes by induction on $\kappa$. 
The result is trivial for $\kappa=0$, so
we assume that $\kappa \geq 1$.
We will change notation somewhat.
Let $p_2/q_2=p/q$ and let
$p_1/q_1=p'/q'$, the even predecessor
of $p_2/q_2$.  Define
\begin{equation}
p_3=p_2-2p_1, \hskip 30 pt
q_3=q_2-2q_1.
\end{equation}
Then
$\kappa_3=\kappa_2-1$.  It suffices to
prove that
$\omega_2-2\tau_2=\omega_3-2\tau_3$.
This is what we will do.

We have
$$w_3=\omega_2-4\tau_2.$$
We define $u_3=3\tau_2-w_2$.  Note that
$\omega_2-2\tau_2=\omega_3-2u_3$.
So, to finish the proof, we just have
to check that $u_3=\tau_3$.  By hypothesis,
we have $u_3>0$.  Since 
$0<\omega_2-2\tau_2=\omega_3-2u_3$, we have
$u_3 \in (0,\omega_3/2)$.  So, we just have
to check that $2p_3u_3 \equiv \pm 1$ mod $\omega_3$.
We will consider the case when $2p_2\tau_2 \equiv 1$ mod $\omega_2$.
The other case works the same way.

In the case at hand, we have
$$k_2=\frac{2p_2\tau_2-1}{\omega_2}.$$
Using this equation, we compute
$$N:=\frac{2p_3u_3-1}{\omega_3}=
\frac{-3-2p_2^2-2p_2q_2 + 6p_2\tau_2}{\omega_2}.$$
Plugging in the equation
$6p_2\tau_2=3+3k_2\omega_2$ and factoring, we
see that $N$ is an integer.  Hence
$2p_3u_3 \equiv 1$ mod $\omega_3$.

\subsubsection{Statement 6}

When $\kappa=0$,
Statement 1
says that either
$\tau=\tau'$ or $\tau+\tau'=\omega'$.
Also, from Equation \ref{zoop} we see that
$2\omega'<\omega$ if and only if
$\tau>\omega/4$.

Suppose that
$\tau'=\tau$ and
$\tau>\omega/4$.
We have $$\tau'=\tau>\omega/4>\omega'/2.$$ which 
contradicts the fact that $\tau'<\omega'/2$.
Suppose that
$\tau'=\omega'-\tau$ and
$\tau<\omega/4$.
We have
$$2\tau'=2\omega'-2\tau>\omega-2\tau=\omega,$$
which again is impossible.

\subsubsection{Statement 7}

We have
$$\widehat \omega=\omega-2\kappa \omega'=
\omega - 2\kappa(\omega-2\tau)=
(1-2\kappa)\omega + 4\kappa \tau.$$
Using this equality, we see that
Statement 7 is equivaent to the truth of
\begin{equation}
\label{refo2}
\frac{\tau}{\omega}<\frac{4\kappa^2-2\kappa+3}{8\kappa^2}.
\end{equation}
By definition
$$
\frac{\tau}{\omega}<\frac{\kappa+1}{2\kappa+3}.
$$
Moreover,
$$\bigg(\frac{4\kappa^2-2\kappa+3}{8\kappa^2}\bigg)
-\bigg(\frac{\kappa+1}{2\kappa+3}\bigg)=\frac{9}{8\kappa^2(2+2\kappa)}>0.
$$
Therefore, Equation \ref{refo2} holds.

\subsubsection{Statement 8}

\startproof
Since $\kappa'\geq 1$, we have
$2\omega^*<\omega'<\omega'+2\tau^*.$
But then
$$\omega^*<\omega'-\omega^*+2\tau^*=2\tau' \leq 2 \tau.
$$
The equality is Statement 5.
The last inequality Statement 7.
Adding $\omega'$ to both sides of this last equation gives
$$\omega^*+\omega'<\omega'+2\tau=\omega.$$
The last equality is Equation \ref{zoop}.
\endproof

\subsection{Existence of the Predecessor Sequence}

We begin by proving the existence of
an auxiliary sequence.  The notation
$p'/q' \leftarrow p/q$ means that
$p'/q'$ is the even predecessor of $p/q$.

\begin{lemma}
\label{weak}
Let $A \in (0,1)$ be irrational.
There exists a sequence
$\{p_n/q_n\}$ converging to
$A$ such that
$p_n/q_n \leftarrow p_{n+1}/q_{n+1}$
for all $n$.
\end{lemma}

\startproof
Let $\H^2$ denote the upper half-plane model
of the hyperbolic plane.
We have the usual Farey
triangulation of $\H^2$ by
ideal triangles.  The geodesics
bounding these triangles join
rationals $p_1/q_1$ and $p_2/q_2$
such that $|p_1q_2-p_2q_1|=1$.
We call these geodesics the
{\it Farey Geodesics\/}.
Two of the Farey geodesics in the tiling
join the points $0/1$ and $1/1$ to $1/0$.
This last point is interpreted as the
point at infinity in the upper half
plane model of $\H^2$.  Let
$Y=\{(x,y)|\ 0<x<1\}$ be the
open portion of $\H^2$ between these
two vertical geodesics.

Each Farey geodesic in $Y$ which joins
two even rationals $p/q$ and $p'/q'$ 
can be oriented
so that it points from $p/q$ to $p'/q'$ if
and only if $p'/q' \leftarrow p/q$.
We leave the rest of the Farey geodesics
unoriented.

We claim that there is a backwards 
oriented path from
$0/1$ to $A$.  To see this, choose any
sequence of even rationals converging to $A$
and consider their sequence of even predecessors.
This gives us a sequence of finite directed
paths joining $0/1$ to rationals which
converge to $A$.  
Given the local finiteness
of the Farey triangulation -- meaning that
any compact subset of $\H^2$ intersects
only finitely many triangles -- we can
take a limit of these paths, at least on
a subsequence, and get a directed path
converging to $A$.  

Reading off the
vertices of this path gives us a
sequence $\{p_n/q_n\}$ with
$p_n/q_n \leftarrow p_{n+1}/q_{n+1}$
for all $n$.
\endproof

\noindent
{\bf Proof of Lemma \ref{neat}:\/}
We get the predecessor sequence from the
sequence in Lemma \ref{weak} in
the following way.  Before each
term $p_n/q_n$ with $\kappa_n \geq 1$
we insert the rational $\widehat p_n/\widehat q_n$.
This is the core predecessor of $p_n/q_n$.
We know from the lemma above that
$\widehat \kappa_n=0$ and that
$p_{n-1}/q_{n-1}$ is the predecessor
of $\widehat p_n/\widehat q_n$. In short
$$p_{n-1}/q_{n-1} \prec \widehat p_n/\widehat q_n \prec p_n/q_n.$$
Once we make all these insertions, the
resulting sequence is a predecessor sequence which
converges to $A$.  Again, we will not stop
to prove uniqueness because we don't care
about it.
\endproof

\subsection{Existence of the Approximating Sequence}

We call the sequence from Lemma \ref{weak} the
{\it even predecessor sequence\/}.  As we
have just remarked, the even predecessor
sequence is a subsequence of the predecessor sequence.

\begin{lemma}
\label{neat1}
Let $\{p_n/q_n\}$ be the
even predecessor sequence
which converges to $A$.
There are infinitely many
values of $n$ such that
$\tau_{n+1}>\omega_{n+1}/4$.
\end{lemma}

\startproof
If this lemma is false, then we might
chop off the beginning and assume that
this never happens. 
We have the formula 
$\omega_n=\omega_{n+1}-2\tau_{n+1}$.
So, if this lemma is false then
we have $2\omega_n<\omega_{n+1}$ only
finitely often.   Chopping off
the beginning of the sequence, we
can assume that this never occurs.

We never have $2\omega_n=\omega_{n+1}$
because $\omega_{n+1}$ is odd.  So, we
always have $\omega_n>\omega_{n+1}$.
In this case, we
have $$r_{n-1}=2r_n-r_{n+1}$$ for
$r \in \{p,q\}$.  Applying this iteratively,
we get that $r_{k}=(k+1)r_1-kr_0$ for $k=1,2,3,...$.
But then $\lim p_n/q_n=(p_1-p_0)/(q_1-q_0)$, which
is rational. This is a contradiction.

Now let $p_n/q_n$ be a term with
$2\omega_n<\omega_{n+1}$.
We will consider the case when $p_n/q_n<p_{n+1}/q_{n+1}$.
The other case has a similar treatment.
We introduce the new rational
$$p_n^{*}/q_n^{*}=\frac{p_{n+1}-p_n}{q_{n+1}-q_n}.$$
Note that the three rationals
$p_n/q_n$ and $p_{n+1}/q_{n+1}$ and
$p_n^{*}/q_n^{*}$ form the vertices of a
Farey triangle.  Moreover $p_{n+1}/q_{n+1}<p_n^*/q_n^*$
because $p_{n+1}/q_{n+1}$ is the Farey sum of
$p_n/q_n$ and $p_n^*/q_n^*$.

Given the geometry of the Farey graph, we have
$$A \in [p_n/q_n,p_n^*/q_n^*].$$
Moreover
$$|p_n/q_n-p_n^*/q_n^*|=\frac{1}{q_nq^*_n} \leq
\frac{1}{q_n^2}<\frac{4}{\omega_n^2}.$$
The second-to-last inequality comes from the
fact that $q_n^*>q_n$.
\endproof

\noindent
{\bf Proof of Lemma \ref{strong0}:\/}
Let $\{p_k/q_k\}$ be the even predecessor
sequence.  If it happens infinitely often that
$\kappa_k \geq 1$ then there are infinitely
many core terms in the predecessor sequence.
Otherwise
the predecessor sequence and the even predecessor
sequence have the same tail end.  But then
the previous result shows that there are
infinitely many values of $k$ for which
$2\omega_k<\omega_{k+1}$.  This gives
infinitely many strong terms.
Suppose that $p/q, p^*/q^*$ are two
consecutive terms in the predecessor sequence,
with $p/q$ non-weak.
\newline
\newline
{\bf Case 1:\/}
Suppose that $p/q$ and $p^*/q^*$ are
both terms in the even sequence.
Then $p/q \leftarrow p^*/q^*$ and
$\tau_*>\omega_*/4$.  But then
$2\omega<\omega_*$, as in 
the proof of Lemma \ref{neat1}.
From here, we get the Diophantine estimate
from Lemma \ref{neat1}.
\newline
\newline
{\bf Case 2:\/}
Suppose that neither $p/q$ not $p^*/q^*$
are terms in the even sequence.  This
case cannot happen because when
$p^*/q^*$ is the core predecessor of
some rational and $p/q$ is the core
predecessor of $p^*/q^*$.  This
contradicts Statement 4 of Lemma \ref{omnibus}.
\newline
\newline
{\bf Case 3:\/}
Suppose that $p/q$ is a term of the
even sequence but $p^*/q^*$ is not.
Then the term in the predecessor sequence
after $p^*/q^*$ is $p^{**}/q^{**}$,
which belongs to the even sequence.
By Statement 3 of
Lemma \ref{omnibus}, we have
$p/q \leftarrow p^{**}/q^{**}$.
Moreover $2\omega<\omega^*<\omega^{**}$.
From here, we get the Diophantine estimate
from Lemma \ref{neat1}.
\newline
\newline
{\bf Case 4:\/}
Suppose that $p/q$ is not a term in
the even sequence but $p^*/q^*$.
Let $p'/q'$ be the term preceding
$p/q$ in the predecessor sequence.
By Statement 4 of Lemma \ref{omnibus},
we see that $p'/q' \leftarrow p/q$.
In particular, $\kappa(p/q)=0$ and
$\tau<\omega/3$.  Using the formula
$\omega'=\omega-2\tau$, we see that
$3\omega'>\omega$.  At the same time
$\omega'<\omega<2\omega^*$.  Lemma
\ref{neat1} gives us
$$\bigg|A-\frac{p'}{q'}\bigg|<
\frac{4}{(\omega')^2}<\frac{36}{\omega^2}.$$
At the same time
$$\bigg|\frac{p}{q}-\frac{p'}{q'}\bigg| =
\frac{1}{qq'}<\frac{4}{\omega \omega'}<\frac{12}{\omega^2}.$$
The result in this case then follows from
the triangle inequality.
\endproof

\subsection{The Capacity of a Certain Line}

Let $p/q$ be an even rational parameter
with $\kappa \geq 1$.  Let
$\widehat p\widehat q$ be the core
predecessor of $p/q$.  In this section
we prove 

\begin{lemma}
\label{nocross3}.
The line $x=\widehat \tau$
has capacity $4\kappa+2$ with respect
to $p/q$. 
\end{lemma}

Suppose that $x=\nu$ is
the line capacity $4\kappa+2$ which
is closest to the $y$-axis.
Let $\mu=\omega-2\tau$.

\begin{lemma}
\label{nocross2}
$(2\kappa+1) \mu+2\nu=\omega$
and $\nu<\mu$.
\end{lemma}

\startproof
Define
\begin{equation}
F_{\kappa}=\frac{\kappa}{2\kappa+1}.
\end{equation}
Let $F$ be the union of all such
rationals.

We rescale the first block so that it
coincides with the unit square.
This rescaling amounts to dividing by
$\omega$. For each quantity $\lambda$
defined above,
we let $\lambda^*=\lambda/\omega$.
Within the unit square, our identity
and our inequality become
\begin{equation}
\label{id2}
(2\kappa+1) \mu^*+2\nu^*=1, \hskip 30 pt
\nu^* < \mu^*.
\end{equation}
The rescaled horizontal and
vertical lines depend continuously
on the parameter $\tau^*$.
Moreover, when $\tau^* \in (F_{\kappa},F_{\kappa+1})$
is rational,
all the horizontal and vertical lines of
capacity up to $4\kappa+2$ are distinct,
because the denominator of the corresponding
rational is at least $2\kappa+1$.
Therefore, the quantity $\kappa$ is a locally
constant function of $\tau^*$, and
changes values only when $\tau^*$
passes through a value of $F$.

Consider what happens when $\tau^*=F_{\kappa}+\epsilon$,
and $\epsilon \in (0,F_{\kappa+1}-F_{\kappa})$.
We compute
\begin{equation}
\label{derive2}
(2\kappa +1)\tau^* - \kappa = (2\kappa +1) \epsilon<1/2
\end{equation}
Hence, by definition, the barrier line
is the line $x=(2\kappa+1)\epsilon$. Hence
\begin{equation}
2\nu^* = (4 \kappa +2) \epsilon.
\end{equation}
We also have
\begin{equation}
\mu^*=1-2\tau^*.
\end{equation}  
But now we compute easily that
Equation \ref{id2} holds for
all $\epsilon \in (0,F_{\kappa+1}-F_{\kappa})$.
\endproof

In view of Lemma \ref{nocross2}, we just
have to prove that
\begin{equation}
\label{goal5}
(2\kappa+1)(\omega-2\tau) + 2\widehat \tau = \omega
\end{equation}
By Statement 5 of Lemma \ref{omnibus} we have
$\omega-2\tau = \widehat \omega-2\widehat \tau$.
But then Equation \ref{goal5} is equivalent to
\begin{equation}
\label{goal6}
(2\kappa+1)\widehat \omega - 4\kappa \tau = \omega.
\end{equation}
This equation holds, because
$$\omega-\widehat \omega=
2\kappa \omega'=2\kappa(\omega-2\tau)=
2\kappa(\widehat \omega-2\widehat \tau)=
2\kappa \widehat \omega-4\kappa \widehat \tau.$$
This completes the proof.



\end{document}




\newpage

==> Backup/6box.tex <==

\section{The Box Lemma}

\subsection{Trivial Cases}

We fix $p/q$. We check the Box Lemma for
$p/q=1/2$ by hand, and henceforth
assume that $p/q \not = 1/2$.

By construction, $\Gamma$ can only intersect
$\partial R$ in the right edge, which we call $\rho$.
Suppose that $\Gamma$ intersects $\rho$ exactly twice.
Because $\Gamma$ is a closed loop,
we conclude that
the portion of $\Gamma$ contained in $R$ is
an arc whose endpoints are on $\rho$.
So, we just have to show that $\Gamma$ always
intersects $\rho$ exactly twice.

We first take care of some trivial cases of the
lemma. If $\rho$ has capacity $2$, then
$\Gamma$ can intersect $\rho$ at most twice,
and the large $x$-diameter of $\Gamma$
implie that $\Gamma$ does intersect $\rho$.
By symmetry, $\Gamma$ intersects
$\rho$ twice. 

Now we deal with the case when
$p/1=1/2n$. Here $R$ is a $1 \times \omega$
rectangle, and the line $x=1$ has capacity $4$.
The two lines of capacity $1$ are spaced
one unit apart. Figure 6.1 shows a
representative case.

\begin{center}
\resizebox{!}{2.3in}{\includegraphics{Pix/poly1.8.ps}}
\newline
{\bf Figure 6.1:\/} $\Gamma_{1/8}$ and
auxiliary lines.
\end{center} 

$\Gamma$ cannot cross $\rho$ in between the
two lines of capacity $2$ because this is
just a single segment centered on the horizontal
midline of the first block, and the plaid
model never intersects such segments.
From the topology of closed loops, we
see that $\Gamma$ crosses $\rho$ above the
horizontal midline an odd number of times,
and likewise below the horizontal midline.
(We will give this argument in more detail below.)
Since $\Gamma$ crosses $\rho$ at most $4$
times, we see that $\Gamma$ must cross 
$\rho$ exactly once above the horizontal
midline and once below.
This takes care of the proof for the parameters
$p/q=1/2n$.  

\subsection{The Proof Modulo a Detail}

Suppose now that $p>1$ and
that $\rho$ has capacity $4$.
In this situation $\kappa \geq 1$.
Of the two vertical lines of capacity $\lambda$ we say that
the {\it near one\/} is the one closer to the $y$-axis.
Let $V$ be the line segment contained in the

We define
the {\it barrier line\/} to be the
near line of capacity $4\kappa+2$.
Lemma \ref{nocross} explains the geometric
significance of this line.   At the end
of this chapter, we will show that
the barrier line is the line $y=\widehat \tau$,
where $\widehat \tau$ is the tune of
the core predecessor $\widehat p/\widehat q$.
We let $V$ be the portion of the barrier
line between the two horizontal lines of
capacity $2$.
Below we will prove the following result.

\begin{lemma}
\label{nocross}
$V \subset R$ and
no plaid polygon
intersects $V$
\end{lemma}

Figure 6.2
shows three sub-rectangles
$R_1,R_2,B \subset R$.  The horizontal dividers in 
the picture are the horizontal lines of capacity
$2$.  

\begin{center}
\resizebox{!}{1.8in}{\includegraphics{Pix/box4.eps}}
\newline
{\bf Figure 6.2:\/} The rectangles $R_1,B,R_2$.
\end{center} 

Assume Lemma \ref{nocross} for now.
Since $\Gamma$ does not intersect $V$,
we see that the portion of
$\Gamma$ between the two horizontal lines
of capacity $2$ cannot intersect $\rho$.
Hence, by symmetry, it suffices to
prove that $\Gamma$ intersects the
right edge $\rho_1$ of $R_1$ exactly once.

We know that $\Gamma$ cannot intersect
$\rho_1$ more than twice because then,
by symmetry, $\Gamma$ would intersect
$\rho$ at least $6$ times.
If $\Gamma$ intersects $\rho_1$ exactly
twice, then $\Gamma$ is trapped in
$R_1$ and cannot get around to close up
with the portion of $\Gamma$ outside $R_1$.
Since $\Gamma$ cannot get trapped in this way,
we see that $\Gamma$ intersects $\rho_1$
at most once.  On the other hand,
if $\Gamma$ does not intersect
$\rho_1$ at all, then $\Gamma$ is
trapped in the same way. In short,
$\Gamma$ intersects $\rho_1$ exactly
once, and the same goes for $\rho_2$.

The rest of the chapter is devoted to
proving Lemma \ref{nocross}.

\subsection{The Blocking Interval}

We define the {\it mass\/} of an integer point on the $y$-axis
to be the mass given to it by the functions $F_P$ and
$F_Q$.  In other words, the mass of a point on the
$y$-axis is the mass of the $\cal P$ and $\cal Q$ lines
which contain that point.  We define the {\it sign\/} of
such a point in the same way.  The two points
$(0,\tau)$ and $(0,\omega-\tau)$ have mass $1$.
One of these two points has the same sign as the
barrier line.  We will give the proof when
$(0,\tau)$ has the same sign as the barrier line.
Also, we will assume that the signs are positive.
The other $3$ cases have essentially the same
treatment as the case we treat.  In each of
these other cases, one swaps the words
{\it positive\/} with {\it negative\/} and/or
turns the entire picture upside down.

So, again, we are assuming that $(0,\tau)$ and
the barrier line have the same sign, and that
this sign is positive.
Let $w$ denote the width of the rectangle $B$ and let
$h=\omega-2\tau$.  Here $h$ is the length of $V$
and also the width of $R$.  Let $U$ denote the
interval of the $y$-axis whose length is
$h+2w$ and whose lower endoint is $(0,\tau)$.
Figure 6.3 shows $U$ and $V$ together.

\begin{center}
\resizebox{!}{2.5in}{\includegraphics{Pix/box5.eps}}
\newline
{\bf Figure 6.3:\/} The intervals $V$ and $W$.
\end{center} 

\begin{lemma}
Suppose that the point of mass $\mu$ is not contained
in the interior of $U$.  Then the $\cal P$ and
$\cal Q$ lines through this point do not
intersect $V$.
\end{lemma}

\startproof
This follows immediately from the fact that
these lines have slope greater than $-2$.
\endproof

\begin{corollary}
Suppose that $U$ contains no points of positive
sign and mass less than $4\kappa+2$.  Then
Lemma \ref{nocross} is true.
\end{corollary}

\startproof
The $\cal P$ and $\cal Q$ lines through such
points are the only ones which could produce
light points on $V$.
\endproof

Below we will prove the following identity:
\begin{equation}
\label{MAIN}
(2\kappa+1) h+2w=\omega.
\end{equation}
We will also prove that $w \leq h$, so that $V \subset R$.

Let's see how Equation \ref{MAIN} finishes the
proof.  The masses occur on the $y$-axis in
an arithmetic progression, modulo $\omega$.
Since \begin{itemize}
\item $(0,\omega-\tau)$ has mass $1$ and
negative sign, and
\item $(0,\tau)$ has mass $1$ and positive sign,
\item $h=(\omega-\tau)-\tau$,
\end{itemize}
the points on the $y$-axis having
positive sign and mass $2\lambda+1$,
at least for $\lambda=1,...,2\kappa$, are
\begin{equation}
(0,\tau-\lambda h)+(0,\omega \Z).
\end{equation}
The second summand is included just so that we remember
that the whole assignment of masses is invariant under
translation by $(0,\omega)$.  Also, we say ``at least''
because once $\lambda$ is large enough the sign will
change.

Thanks to Equation \ref{MAIN}, we have
$$\tau-2\kappa h =
\tau-(2\kappa+1)h +h =
\tau-(\omega-2w)+h=-\omega+\tau+h+2w.$$
Therefore, for $\lambda=1,...,2\kappa$, the numbers
$\tau-\lambda h$ all lie in the interval
\begin{equation}
[-\omega + \tau+h+2w,\tau].
\end{equation}
In particular, the translates of the corresponding
points by $(0,\omega\Z)$ are all disjoint from
our interval.  Hence, no $\cal P$ or $\cal Q$ line
of positive sign and mass less than $4\kappa+2$
can intersect $V$.  This finishes the proof of
the Box Lemma, modulo Equation \ref{MAIN} and
the inequality $w \leq h$.

In the next two sections, we will establish
Equation \ref{MAIN} and also the inequality
$w<h$.  We will include one last section which
elaborates on the argument given above.
This elaboration will be useful in \S 9.

\subsection{Proof of the Identity}

Now we prove Equation \ref{MAIN}.
Define
\begin{equation}
F_{\kappa}=\frac{\kappa}{2\kappa+1}.
\end{equation}
Let $F$ be the union of all such
rationals.

We rescale the first block so that it
coincides with the unit square.
This rescaling amounts to dividing by
$\omega$. For each quantity $\lambda$
defined above,
we let $\lambda^*=\lambda/\omega$.
Within the unit square, our identity
is
\begin{equation}
\label{id2}
(2\kappa+1) h^*+2w^*=1.
\end{equation}
The rescaled horizontal and
vertical lines depend continuously
on the parameter $\tau^*$.
Moreover, when $\tau^* \in (F_{\kappa},F_{\kappa+1})$
is rational,
all the horizontal and vertical lines of
capacity up to $4\kappa+2$ are distinct,
because the denominator of the corresponding
rational is at least $2\kappa+1$.
Therefore, $\kappa$ is a locally
constant function of $\tau^*$, and
changes only when $\tau^*$
passes through a value of $F$.

Consider what happens when $\tau^*=F_{\kappa}+\epsilon$,
and $\epsilon \in (0,F_{\kappa+1}-F_{\kappa})$.
We compute
\begin{equation}
\label{derive2}
(2\kappa +1)\tau^* - \kappa = (2\kappa +1) \epsilon<1/2
\end{equation}
Hence $w=(2\kappa+1)\epsilon$, which means that
$2w^* = (4 \kappa +2) \epsilon$.
We also have
$h^*=1-2\tau^*$.
From these equations one can easily compute that
Equation \ref{id2} holds for
all $\epsilon \in (0,F_{\kappa+1}-F_{\kappa})$.

\subsection{A Related Result}

We first deal with a minor technical point.

\begin{lemma}
\label{triv}
$3\widehat \tau<\widehat \omega$.
\end{lemma}

\startproof
Since $\widehat p/\widehat q$ is assumed
to be the nontrivial core predecessor of
$p/q$, Statement 4 of Lemma \ref{omnibus}
gives $\widehat \kappa=0$.  This forces
$3\widehat \tau \leq \widehat \omega$.
The case of equality would force
$\widehat p/\widehat q=1/2$.  But
then the even predecessor of
$p/q$ would be the even predecessor of
$1/2$, by Statement 3 of Lemma \ref{omnibus}.
This is not possible.
\endproof

Now we come to the result of interest to us.

\begin{lemma}
\label{core1}
Let $\Omega$ be the vertical interval
of length $\widehat \omega$ and
centered at the point $(0,\omega/2)$.
The only points of mass less than
$4\kappa+2$ contained in $\Omega$ are
the points of mass $1$.
\end{lemma}

\startproof
We will give the proof when the sign
of $(0,\tau)$ is positive.  The other
case is essentially the same.  Since
$\Omega$ is symmetrically placed with
respect to the horizontal midline of the
first block $[0,\omega]^2]$, it suffices
to show that $\Omega$ does not contain
any points of positive sign and mass
$3,5,7,...,4\kappa+1$.  

The endpoints of $\Omega$ are
$$(0,\omega/2-\widehat \omega/2), \hskip 30 pt
(0,\omega/2+\widehat \omega/2).$$
As in our
proof of the Box Lemma, it suffices to prove that
the points
$$\tau-\lambda h, \hskip 30 pt
\lambda=1,...,2\kappa$$
lie in the interval
$$[-\omega/2+\widehat \omega/2,\omega/2-\widehat \omega/2].$$
Since these points occur in linear order, it suffices to prove
the following two inequalities:
\begin{equation}
\label{MAIN2}
\tau-h<\omega/2-\widehat \omega/2, \hskip 30 pt
\tau-2\kappa h>-\omega/2+\widehat \omega/2.
\end{equation}

Since $h=\omega-2\tau$, the first identity
is equivalent to
$$3\omega-6\tau>\widehat \omega.$$
But, by Statement 5 of Lemma \ref{omnibus}, 
$$3\omega-6\tau=3\widehat \omega-6\widehat \tau.$$
But the inequality
$$3\widehat \omega-6\widehat \tau>\widehat \omega.$$
is the same as the one proved in Lemma \ref{triv}.
This takes care of the first inequality.

We already know that
$$\tau-2\kappa h=-\omega+\tau+h+2w.$$ Hence,
the second inequality is the same as
\begin{equation}
\label{final}
(-\omega+\tau+h+2w)-(-\omega/2+\widehat \omega/2)>0.
\end{equation}
Plugging in $h=\omega-2\tau$ and $w=\widehat \tau$,
and using the relation $\omega-2\tau=\widehat \omega-2\widehat \tau$,
we see that the left hand side of Equation
\ref{final} is just $\widehat \tau$.
\endproof

\noindent
{\bf Remark:\/} As a byproduct of our proof we note that
the points $(0,\tau)$ and $(0,\tau+h+2w)$ have the same sign.
Also, $h+2w=\widehat \omega$. 



\newpage



==> Backup/6copy.tex <==
\section{The Arc Copying Theorem}

\subsection{A Big Polygon}

Let $p/q$ be an even rational parameter
and let $\omega=p+q$. 
Define the $x$-{\it diameter\/} of a set
to be the diameter of the projection of
the set onto the $x$-axis. Here is a
result from [{\bf S0\/}] which we
repeat here.

\begin{theorem}
\label{first}
Let $B$ denote the first block.
Then there exists a plaid polygon
in $B$ whose $x$-diameter is at least
$\omega^2/(2q)-1$.  Moreover,
this polygon has bilateral symmetry
with respect to reflection in the
horizontal midline of $B$.
\end{theorem}

\startproof
Let $L$ be the horizontal
line of capacity $2$ and positive sign
which intersects $B$. Let $y$ be
such that $(0,y) \in L$.  Define
\begin{equation}
z_1=(0,y) \in L, \hskip 30 pt
z_2=(\omega^2/2q,y).
\end{equation}
A calculation shows that
\begin{equation}
F_P(z_1)=F_Q(z_1)=F_Q(z_2)=1.
\end{equation}
Hence $z_1$ and $z_2$ are two
light points on $L$.  By
Theorem \ref{hier}, they are
the only two light points on $L$.

By definition, there is a plaid polygon
$\Gamma$ which crosses the unit horizontal
edge having $z_1$ as its left endpoint.
Since $\Gamma$ is closed, $\Gamma$ must
cross $L$ twice.  But then $\Gamma$ must
cross $L$ in the unit horizontal segment
containing $z_2$.
This gives the lower bound on the $x$-diameter.

Let
$\Gamma'$ denote the reflection
of $\Gamma$ in the horizontal midline of $B$.
We want to show that $\Gamma'=\Gamma$.
Let $V_1$ and $V_2$ denote the two vertical lines
of $B$ having capacity $2$.  These lines are 
symmetrically placed with respect to the
vertical midline of $B$.  Hence, one of the
two lines, say $V_1$, lies less than $\omega /2$
units away from the $y$-axis.
Since 
$\omega /2<\omega^2/(2q),$
the point $z_2$ is separated from the $y$-axis by $V_1$.
Hence both $\Gamma$ and $\Gamma'$ intersect
$V_1$.  Since there can be at most $1$
plaid polygon which intersects $V_1 \cap B$,
we must have $\Gamma=\Gamma'$.
\endproof

We define the {\it special points\/} of $\Gamma$ to
be the intersection points of the vertical line $x=1/2$ and
the two horizontal lines of capacity $2$.
We call these special points $S_+\Gamma$ and
$S_-\Gamma$.
Referring to the proof above, we have
\begin{equation}
S_+\Gamma=z_1+(1/2,0), \hskip 30 pt
S_-\Gamma=(1,\omega)-S_+\Gamma.
\end{equation}
Figure 4.1 shows the polygon for
the parameter $5/12$.


\begin{center}
\resizebox{!}{4.5in}{\includegraphics{Pix/big5.12.ps}}
\newline
{\bf Figure 4.1:\/} The big polygon for the parameter $5/12$.
\end{center}

Figure 4.1 also shows the lines of capacity $0$ and $2$.
The lines of capacity $0$ form the boundary of the block.
The two special points just
mentioned lie on the left side of the two horizontal
lines of capacity $2$.
The left vertical line $V$ of capacity $2$ divides
$\Gamma$ into two halves,
$L\Gamma$ lies to the left of $V$
and $R\Gamma$ lies to the right of $V$
The endpoints of these two arcs lie on the
unit vertical segments of $V$ containing the two
light points.

At this point it seems that one could take a
sequence $\{p_k/q_k\}$ which converges to
the limit parameter $A$, and take a
geometric limit involving the ever-growing
polygons $\Gamma_k$.  This is what we will
ultimately do, but it needs to be done carefully.
The problem is that it is hard to guarantee
that the limiting polygon corresponds to a
well-defined orbit in the PET.
The reader who wants to see what goes wrong
with the simplest attempt can skip ahead
to \S \ref{fail}.  The geometric result
proved below turns out to be key tool
needed to make the limiting argument work.

\subsection{Some Definitions}

\noindent
{\bf Red and Blue Parameters:\/}
We call a rational parameter $p/q$
{\it red\/} if $a<\omega/2$.
Here $a$ solves the congruence
$2ap \equiv -1$ mod $\omega$.  Otherwise
we call $p/q$ {\it blue\/}.  These two
cases correspond to whether or not
the horizontal line of mass $1$ lies below
or above the horizontal midline of the first block.
\newline
\newline
{\bf The Width:\/}
For each parameter $p/q$, we let
$\alpha$ be the smaller of the two
solutions to $2\alpha p \equiv \pm 1$ mod $\omega$.
If $p/q$ is red then $\alpha=\omega-a$ and
if $p/q$ is blue then $\alpha=a$.  In either
case, we define the {\it width\/} to be
$\omega-2\alpha$.  This is the vertical
distance between the two horizontal lines
of capacity 2.
\newline
\newline
{\bf Even Predecessors:\/}
Consider two even rational parameters
$p_1/q_1$ and $p_2/q_2$.  We say that
$p_1/q_1$ is the {\it even predecessor\/}
of $p_2/q_2$ if
\begin{equation}
q_1<q_1, \hskip 30 pt
|p_1q_2-p_2q_1|=1.
\end{equation}
It turns out that the even predecessor of any
even rational in $(0,1)$ is unique.
Fractions which have this relationship
are called {\it Farey related\/}.
In this case we write
$p_1/q_1 \to p_2/q_2$.
More generally, we will write
$$p_1/q_1 \to p_2/q_2 \to p_3/q_3 \to ...$$
if every consecutive pair obeys the
rules described above.
\newline
\newline
{\bf Happy and Unhappy Pairs:\/}
Assuming that $p_1/q_1 \to p_2/q_2$, we
call the pair $(p_1/q_1,p_2/q_2)$ 
{\it happy\/} if either both are red
or both are blue.  Otherwise, we call
them {\it unhappy\/}. 

\subsection{The Main Result}

Suppose $p_1/q_1 \to p_2/q_2$.
Let $\Gamma_1$ and $\Gamma_2$ be the two big
polygons corresponding to $p_1/q_1$ and $p_2/q_2$
respectively.  Let $\delta_j$ denote the
width of $p_j/q_j$.

\begin{theorem}[Arc Copying]
Let $p_1/q_1 \to p_2/q_2$.  
$L\Gamma_2$ contains two vertically
translated copies of $L\Gamma_1$.
In the happy case, the translation
distance between the two copies is
$\delta_2-\delta_1$.  In the
unhappy case, the translation
distance is $\delta_2+\delta_1$.
\end{theorem}

Figures 4.2 and 4.3 respectively show 
examples of the happy case and the unhappy case.
In the happy case it can happen that the two
translated copies of $\Gamma_1$ overlap.

\begin{center}
\resizebox{!}{1.7in}{\includegraphics{Pix/big2.5.ps}}
\resizebox{!}{3.4in}{\includegraphics{Pix/big7.18.ps}}
\newline
{\bf Figure 4.3:\/} Arc copying for $2/5 \to 7/18$.
\end{center}

\begin{center}
\resizebox{!}{1.8in}{\includegraphics{Pix/big5.12B.ps}}
\resizebox{!}{3.5in}{\includegraphics{Pix/big12.29.ps}}
\newline
{\bf Figure 4.2:\/} Arc copying for $5/12 \to 12/29$.
\end{center}


The significance of the Arc Copying Theorem
is that it guarantees that $\Gamma_2$ comes
close to the $y$-axis not just at its
two special points but also at certain
translates of the special points of $\Gamma_1$.
When this reasoning is applied iteratively,
we will get a huge supply of points where
our big polygons come close to the $y$-axis.
For example, we have the longer chain
$$1/2 \to 2/5 \to 5/12 \to 12/29,$$
and this explains why
$\Gamma(12/29)$ seems to come close to the
$y$-axis in $16=2^4$ points.
These $16$ points seem to be arranged into a kind
of ''finite binary Cantor set''.  In \S 5 we will
formalize this idea by defining the notion of
a {\it binary cluster\/} of $2^n$ points.

\subsection{Proof in the Happy Case}

We will first give the proof of the Arc Copying
Theorem in the happy case.  The proof in the unhappy
case is almost the same, but there is a
technical point that needs to be cleared up.
We will also assume that both parameters
are red, so that their horizontal lines
of capacity $2$ lie above the $x$-axis.
The blue-blue case is the same except
for a global sign change.

We will show that $L\Gamma_2$ contains a 
vertical translate $T_+(L\Gamma_1)$ where
\begin{equation}
T_+(S_+\Gamma_1)=S_+\Gamma_2.
\end{equation}
By reflection symmetry,
$L\Gamma_2$ contains a second translated
$T_-(L\Gamma_1)$ where
\begin{equation}
T_-(S_-\Gamma_1)=S_-\Gamma_2.
\end{equation}
The difference in the vertical translations between
these two maps is $\delta_2-\delta_1$.

let $B_j$ denote the first block for the
parameter $p_j/q_j$.    Let
$R_j \subset B_j$ denote the region to the
left of the left vertical line of capacity $2$.
The region of interest to us is
\begin{equation}
T_+(R_1).
\end{equation}
This region has length $\omega_1$ and width
$\alpha_1$.  Again $\alpha_1$ is the smaller
of the two solutions to $2p_1\alpha_1 \equiv \pm 1$ mod $\omega_1$.
Figure 4.3 shows a schematic picture of
$B_2$ and $T_+(R_1)$.  The region
$T_+(R_1)$ is shaded. 


\begin{center}
\resizebox{!}{3.5in}{\includegraphics{Pix/copy1.eps}}
\newline
{\bf Figure 4.4:\/} The region $T_+(R_1)$.
\end{center}

Figure 4.4 shows the case where
$T_+(R_1) \subset R_2$.  We will
first consider this case, and then
explain the modifications needed to
handle the possibility that
$T_+(R_1) \not \subset R_2$.
In the case at hand, we will show that
the portion of the plaid tiling with respect to
$p_2/q_2$ inside $T_+(R_1)$ is just a translated
copy of the corresponding portion of the
plaid tiling with respect to $p_1/q_1$ inside
$R_1$.   

We consider the horizontal intersection points
first.  Let $z_2$ be an intersection point,
contained on some horizontal unit segment
$h_2 \subset T_+(R_1)$.  Let $h_1=T_+^{-1}(h_2) \subset R_1$.
Because the rectangle $T_+(R_1)$ is more than twice
as tall as it is wide, there is some line $G_2$ in
one of the $4$ families ${\cal P\/}_+$,
${\cal P\/}_-$, ${\cal Q\/}_+$, ${\cal Q\/}_-$
such that
\begin{itemize}
\item $q_2$ is at the intersecton of $G_2$ and
the horizontal line $H_2$ containing $h_2$.
\item The $G_2$ and $H_2$ both intersect the
$y$-axis inside $T_+(R_2)$.
\end{itemize}
See \S \ref{pos} for a definition of these families.
Figure 4.5 shows what we have in mind.

\begin{center}
\resizebox{!}{3.5in}{\includegraphics{Pix/copy2.eps}}
\newline
{\bf Figure 4.5:\/} An intersection point in $T_+(R_1)$.
\end{center}

Let $Y$ denote the $y$-axis.
Let $G_1$ be the line from the same family (with respect
to $p_1/q_1$, which contains the intersection point
$T_+^{-1}(G_2 \cap Y)$.  Define $H_1$.  Define
$z_1=G_1 \cap H_1$.  Note that $T_+(z_1)$ probably
does not equal $z_2$, because $z_1$ is an intersection
point relative to the parameter $p_1/q_1$ and $
z_2$ is an intersection point with respect to 
$p_2/q_2$.  Nevertheless, we will establish a
close correspondence between these points.

\begin{lemma}
$z_1$ lies in the unit horizontal interval $h_1$ which
has the property that $T_+(h_1)=h_2$.
\end{lemma}

\startproof
Consider the point $z_1'=T_+^{-1}(z_2)$.  We
certainly have $z_1' \in h_1$.
There are $4$ cases, depending on which family
of lines is involved.  The points
$z_1,z_1',z_2$ all have the same type.

Suppose first that they have type ${\cal P\/}_-$.
Our result is trivial if all these points
all lie on $Y$.  So, we can assume that they
all lie to the right of $Y$.  In this case,
The distance from $z_1'$ to the endpoint
of $h_1$ is at least 
$$1/P_2.$$
The line
$z_1'$ lies on a line of slope $-P_2$ through
the same point as the line of slope $-P_1$
which contains $z_1$.  Since
$p_1/q_1 \to p_2/q_2$, the difference
in these slopes is
$$|P_1-P_2|=|\frac{2p_1\omega_2-2p_2\omega_1}{\omega_1\omega_2}=
\frac{2}{\omega_1\omega_2}.$$
Both points lie within $\omega_1/2$ from $Y$. Therefore
$$|z_1-z_1'|<\frac{2}{\omega_1\omega_2} \times \frac{\omega_1}{2}<
\frac{1}{\omega_2}<\frac{1}{P_2}.$$
Hence both $z_1$ and $z_1'$ lie on the unit horizontal
interval, which must be $h_1$.

The proof works the same way for the other $3$ line types.
\endproof

\begin{lemma}
If $z_2$ is a light point with respect to
$p_2/q_2$ then $z_1$ is a light point with
respect to $p_1/q_1$.
\end{lemma}

\startproof
Let $\gamma_j$ and $\eta_j$ be the $y$-intercepts
of the lines $G_j$ and $H_j$ containing the point $z_j$.
To say that $z_j$ is a light point is to say that
\begin{equation}
|[P_j\gamma_j+1]_2|<
|[2P_j\eta_j]_2|,
\end{equation}
and that these two expressions have the same sign.
So, we will assume that this is true for
$j=2$ and then establish it for $j=1$.

Multiplying through by $\omega_2$, we have the
inequality
\begin{equation}
|[2p_2\gamma_2+\omega_2]_{2\omega_2}|<
|[4p_2\eta_2]_{2\omega_2}|,
\end{equation}
and both expressions have the same sign.
Here the expression $[t]_{2 \omega_2}$ means that
we reduce $t$ mod $2\omega_2$ and take the
value to lie in $(-\omega_2,\omega_2)$.

We have
\begin{equation}
\gamma_1=\gamma_2-a_1+a_2, \hskip 30 pt
\eta_1=\eta_2-a_1+a_2.
\end{equation}































\end{document}




==> Backup/8copy.tex <==
\section{The Weak and Strong Copy Lemmas}

\subsection{Alignment of the Intersection Points}
\label{align}

In this chapter we prove the Weak and Strong
Copy Lemmas.  The two results have essentially
the same proof, except for a few minor details.

Now we explain how the intersection points
inside $\Sigma'$ w.r.t. $p'/q'$ line up with
the intersection points inside $\Sigma$ w.r.t. $p/q$.

We define a {\it slanting line\/} to be either
a $\cal P$ line or a $\cal Q$ line (w.r.t. the
relevant parameter.)
Let $z' \in \Sigma'$ be the intersection point of
a $\cal V$ line $V'$ and a slanting line $L'$
w.r.t. $p'/q'$.
Let $V=V'$ and let $L$ be the slanting line 
w.r.t. $p/q$ which has the same $y$-intercept
as $L'$ and also the same type, $\cal P$ or $\cal Q$.
Note that $L$ and $L'$ are not the same line;
they have different slopes.

Recall that a {\it vertical unit segment\/} is a
vertical edge of an integer unit square.

\begin{lemma}[Alignment]
\label{matrix}
$z$ and $z'$ lie in the same unit vertical segment.
\end{lemma}

\startproof
The difference in slopes of the two lines is
$2/(\omega\omega')$.
Hence
\begin{equation}
\|z-z'\| \leq \frac{2\tau'}{\omega \omega'}<\frac{1}{\omega}<\frac{1}{\omega'}
\end{equation}
But $z'$ is at least
$1/\omega'$ from the interval contaiing it.
Hence $z$ and $z'$ lie in the same vertical unit interval.
\endproof

\noindent
{\bf Remark:\/}
In replacing $1/\omega$ by $1/\omega'$, we threw away
some of the strength of our estimate.  We did this
because in \S 9 we will have a much tighter estimate,
and we want the two arguments to look similar.

\begin{lemma}
\label{vert}
Suppose that $\Sigma \cap \Pi$ and
$\Sigma' \cap \Pi'$ have 
the same intersection with the $\cal V$
lines. Then $\Sigma \cap \Pi=\Sigma' \cap \Pi'$.
\end{lemma}

\startproof
Let $Q'$ be a tile of $\Sigma'$ such that
that $\Pi \cap Q' \not = \Pi' \cap Q'$.
We take $Q'$ to be as low as
possible in $\Sigma'$, so that
the tilings match on on all squares
in $\Sigma'$ below $Q'$.
The two tilings match on the
bottom edge of $Q'$.  They also match
on the left and right edges.  Finally,
the tiles in $Q'$ are determined by how they
intersect $3$ of the $4$ sides.  So, if the
tilings match along at least $3$ of the
$4$ edges of $Q'$, then must also match
along the fourth edge.
\endproof

\subsection{The Mass and Capacity Sequences}
\label{masscap}

We first define a sequence w.r.t. $p'/q'$.
Let $W'$ and $H'$ denote the width and
height respectively of $\Sigma'$.
For indices
\begin{equation}
i=1,...,W', \hskip 30 pt
j=-2W'+1,...,H+2W'+1
\end{equation} 
we define
\begin{equation}
c'_i=[2Pi]_2, \hskip 20 pt
m'_j=[Pj+1]_2.
\end{equation}
When $j\equiv 0$ mod $\omega'$, we have
$m_j=\pm 1$ is only defined up to sign.
We call such an index {\it special\/}.
If $i \not \equiv 0$ mod $\omega'$
then we call $i$ ordinary.

We make all the same definitions w.r.t.
$p/q$, except that we determine the
special indices w.r.t $p'/q'$.  That
is, $j$ is special if and only if
$j' \equiv 0$ mod $\omega'$.

For each index $j$ there is a set $S_j$ of
points $z \in \Sigma$ so that $z$ lies
on a $\cal V$ line of $\Sigma$ and also
on a slanting line whose $y$-intercept
is $(0,j)$.  All these definitions
are taken w.r.t. $p/q$.  By {\it slanting line\/}
we mean a line from one of the $4$ families
considered in the Vertical Lemma from \S 2.

We make all the same definition w.r.t $p'/q'$.
From the alignment of the vertical intersection
points, we know that there is a canonical
bijection between $S_j$ and $S_j'$.  If 
$j$ is a special index, then $S_j'$
consists entirely of dark points. We
call $j$ {\it harmless\/} if $S_j$ also
consists entirely of dark points.

\begin{lemma}[Matching]
Suppose the following is true:
\begin{itemize}
\item $c_i$ and $c_i'$ have the same sign for all $i$.
\item $m_j$ and $m_j'$ have the same sign for all ordinary indices $j$.
\item Every special index is harmless.
\end{itemize}
Then $\Pi \cap \Sigma=\Pi'\cap \Sigma'$.
\end{lemma}

\startproof
Suppose first that $z'$ is some intersection
point on a unit vertical
segment of $\Sigma'$.  Let $z$ be the corresponding
point of $\Sigma$.  Thanks to the Alignment Lemma,
$z$ and $z'$ lie on the same vertical unit segment.
Now $z$ is the intersection of a $\cal V$ line
and a ${\cal P\/}$ line and a ${\cal Q\/}$ line
(for some choice of signs.)  The same goes
for $z'$.  Because all these lines have slope
in $(-2,2)$ and from the way we have chosen
our indices, all these lines have their $y$ intercepts
amongst our list of indices.  

If one of the slanting lines containing $z'$ has
a $y$-intercept which is a special index, then
$z'$ is a dark point.  Since the corresponding
index is harmless, $z$ is also a dark point.
On the other hand, by the Vertical Lemma, we
can determine by looking at the signs of the
relevant lines w.r.t. $p'/q'$ whether $z'$ is
light or dark.  The same goes for $z$. Since
there are no sign changes for the ordinary indices,
we see that $z'$ is light if and only if $z$ is
light.

Now we know that $\Pi \cap \Sigma$ and
$\Pi \cap \Sigma'$ agree on all the vertical sides.
We also know that $\Pi \cap \Sigma$ and
$\Pi \cap \Sigma$ agree along the bottom
edges of these rectangles, because these
edges are in the bottom edge of the first block.
Suppose that there is some unit square
$Q \subset \Sigma=\Sigma'$ where the two tilings
disagree.  We can take $Q$ to be as close to
the bottom edge as possible.  But then 
$\Pi \cap Q$ and $\Pi' \cap Q$ agree on 
the bottom edge of $Q$ and also on the vertical
side edges.  We can determine the tile from
how it intersects $3$ of the sides.  Hence
$\Pi \cap Q=\Pi' \cap Q$ after all.
Since $Q$ is arbitrary, we see that
$\Pi \cap \Sigma=\Pi' \cap \Sigma'$.
\endproof

\subsection{No Sign Changes for the Capacities}
\label{capacityX}

We introduce new variables
\begin{equation}
M_i=M_i\omega, \hskip 30 pt
C_j=c_j\omega, \hskip 30 pt
M_i'=m_i'\omega', \hskip 30 pt
C_j'=c_i'\omega'.
\end{equation}

\begin{itemize}
\item $C_i$ is a nonzero even integer in $(-\omega,\omega)$.
\item $C_i'$ is a nonzero even integer in $(-\omega',\omega')$.
\item $M_j'$ is an odd integer in $[-\omega',\omega']$.
\item $M_j$ is an odd integer in $[-\omega,\omega]$.
\end{itemize}

Let 
\begin{equation}
\lambda= \omega'/\omega.
\end{equation}
We have
\begin{equation}
 C_i'=[2 \omega'  P' i]_{2 \omega'},
\hskip 20 pt
C_i=[2\omega P i]_{2 \omega},
\hskip 20 pt 
\lambda C_i=[2 \omega' P i]_{2  \omega'}.
\end{equation}

We introduce the expression
\begin{equation}
\Psi(i)=|2 \omega Pi - 2 \omega'   P' i|.
\end{equation}
As long as
\begin{equation}
\label{key0}
\Psi(i)<\ell + 2\lambda, \hskip 30 pt
\min(| C_i'|, \omega'-|C_i'|) \geq \ell
\end{equation}
the signs of $ C_i'$ and $C_i$ are the same.

Using the fact that
\begin{equation}
|P-P'|=\frac{2}{\omega\omega'}
\end{equation}
we see that
\begin{equation}
\label{bound0}
\Psi(i)=\frac{4 i}{\omega} \leq \frac{4W'}{\omega}.
\end{equation}

In all cases, we have $W' \leq \tau' \leq \omega'/2$.
Hence $$\Psi(i)<2\lambda<1+2\lambda.$$
So, we can take $\ell=1$ in Equation \ref{key0},
and we see that there are no sign changes for
the capacities.

\subsection{No Sign Changes for the Masses}
\label{masschange1}

We have
\begin{equation}
 M_i'=[\omega'  P' i+\omega']_{2 \omega'},
\hskip 20 pt
M_i=[2\omega P i+\omega]_{2 \omega},
\hskip 20 pt 
\lambda M_i=[ \omega' P i+\omega']_{2  \omega'}.
\end{equation}

We introduce the expression
\begin{equation}
\Xi(i)=|\omega Pi - \omega'   P' i|.
\end{equation}
This function differs from $\Psi$ just in a factor of $2$.
As long as $i$ is an ordinary index and
\begin{equation}
\label{key1}
\Xi(i)<\ell + \lambda, \hskip 30 pt
\min(| M_i'|, \omega'-|M_i'|) \geq \ell
\end{equation}
the signs of $ M_i'$ and $M_i$ are the same.

We have
\begin{equation}
\label{xi}
\Xi(i)=\frac{2i}{\omega}<\frac{2H'+4W'}{\omega}.
\end{equation}
There are several cases to consider.
\newline
\newline
{\bf Case 1:\/}
Suppose that we are in the weak case and
$\tau' \leq 2\omega'-\tau'$. 
We have 
$$H'=\omega'-\tau', \hskip 30 pt
W'=\tau'.$$ 
Using the facts that
$$\tau'=\tau, \hskip 30 pt
\omega'=\omega-2\tau,$$
and plugging the values of $W'$ and $H'$
into Equation \ref{xi}, we get
$$\Xi(i)<\frac{2\omega'+2\tau'}{\omega}=
\frac{2\omega'+2\tau}{\omega}=
\frac{2\omega-2\tau}{\omega}=
\frac{\omega+\omega'}{\omega}=1+\lambda.$$
So, Equation \ref{key1} holds
and there are no sign changes.
\newline
\newline
{\bf Case 2:\/}
Suppose that we are in the weak case and
$\tau'>2\omega'-\tau'$.   This
means that $\tau<\omega/4$ and
$\tau'=\tau$ and $\tau'>\omega'/3$.
We have 
$$H'=2\tau', \hskip 30 pt
W'=\omega-2\tau'.$$
Plugging this into Equation \ref{xi},
we get
$$\Xi(i)<\frac{4\omega'-4\tau'}{\omega}<\frac{8\tau'}{\omega}=
\frac{8\tau}{\omega}<2.$$
So, we only have to worry about the case
when $\widehat C_i=\pm 1$.  This happens
for $i \in \{-\tau',\tau',\omega'-\tau'\}$.
The highest index is $\omega'+\tau'-1$.
we have

$$
\Psi(\pm \tau') \leq
\Psi(\omega'-\tau')=\frac{2\omega'-2\tau'}{\omega}=
\frac{2\omega'-2\tau}{\omega}=\frac{2\omega-4\tau}{\omega}=$$
\begin{equation}
\frac{\omega+(\omega-4\tau)}{\omega}<\frac{\omega+\omega'}{\omega}=1+\lambda.
\end{equation}
So Equation \ref{key1} holds in all cases.
\newline
\newline
{\bf Case 3:\/}
Suppose we are in the strong case and
$\tau' \leq 2\omega'-\tau'$.
We have 
$$H'=\omega', \hskip 30 pt
W'=\tau'.$$
This gives us the estimate
\begin{equation}
\label{bound2}
\Xi(i)<\frac{2\omega'+4\tau'}{\omega}.
\end{equation}
Since $3\tau' \leq \omega'$ and $\tau+\tau'=\omega'$, 
we have
$$2\tau'\leq \omega'-\tau'=\tau.$$
Hence
$$\Xi(i)<\frac{2\omega'+2\tau}{\omega}=
\frac{(\omega'+2\tau)+\omega'}{\omega}=1+\lambda.$$
So, Equation \ref{key1} holds in all cases,
and there are no sign changes.
\newline
\newline
{\bf Case 4:\/}
Suppose we are in the strong case and
$\omega'-2\tau'<\tau'$.  In this case, we have
$$H'=\omega', \hskip 30 pt
W'=\omega'-2\tau'.$$
This gives us the estimate
\begin{equation}
\label{bound3}
\Xi(i)<\frac{6\omega'-8\tau'}{\omega}.
\end{equation}
Using the fact that $\tau+\tau'=\omega'$
and $\tau<\omega/3$, we get
$$\Xi(i)<\frac{6\tau-2\tau'}{\omega}<2.$$
We just have to worry about
$C_i=\pm 1$.  The relevant
indices are $i \in \{-\tau',\tau',\omega'-\tau',\omega'+\tau'\}$.
We have
$$\Psi(\pm \tau') \leq \Psi(\omega'-\tau')<
\Psi(\omega'+\tau') =
\frac{2\omega'+2\tau'}{\omega}<
\frac{\omega+\omega'}{\omega}=1+\lambda.$$
Here we used the fact that $2\omega'<\omega$
and $2\tau'<\omega'$.
So, Equation \ref{key1} holds in all
cases, and there are no sign changes.

\subsection{The Special Indices are Harmless}

To show that our Matching Criterion is satisfied,
we just need to prove that every special
index is harmless.  We will first do this in the
weak case and then in the strong case.

\begin{lemma}
\label{nuisance}
In the weak case
Every special index is harmless.
\end{lemma}

\startproof
Since $H'+2W'<2\omega'$ and $2W'<\omega'$, there
are are at most $2$ special indices, namely
$j=0$ and $j=\omega'$.  For $j=0$ we have
$m_j=\pm \omega$.  This is just the mass w.r.t
$p/q$ of the slanting lines through the origin.
When $j=\omega'$ we compute
\begin{equation}
\label{masschange}
P\omega'+1=P'\omega' + (P-P') \omega' +1 = 2p'+1  \pm
\frac{2}{\omega} \equiv
1 \pm \frac{2}{\omega}  \hskip 10 pt {\rm mod\/}\hskip 5 pt 2\Z.
\end{equation}
In short, $M_j=\omega \pm 2$.

We will consider the case when $M_j=\omega-2$. The
case when $M_j=-(\omega-2)$ has the same treatment.
If $j$ is not harmless than
$C_i=\omega-1$ for some $i=1,...,W$.
From Lemma
\ref{anchor}, we get two cases.
If $\tau$ is odd, then the vertical lines of
capacity $\pm(\omega-1)$ are the lines
$x=(\omega \pm \tau)/2$. Since 
$\tau'=\tau<\omega/3$,
these vertical lines lie outside $\Sigma'$. So,
we don't have to worry about the intersection
point: It does not belong to the set $S_j$.
(We actually have $\tau>\omega/4$ but we
want to use the same argument below in the
Strong Case.)

If $\tau$ is even, then the vertical lies of
capacity $\pm(\omega-1)$ are the lines
$x=\tau/2$ and $x=\omega-(\tau/2)$.
If the line $x=\omega-\tau/2$ has capacity
$\omega-1$ then this line lies outside
$\Sigma'$ and again the intersection point
is irrelevant.

On the other hand, suppose that
the line $x=\tau/2$ has capacity $\omega-1$.
Call this line $V$.
The $\cal Q$ line $L$ corresponding to $M_i$ has
$y$-intercept at least $\omega'$.
Since $L$ has slope greater than $-2$ and
the height of $\Sigma'$ is $\omega'-\tau=\omega'-\tau'$,
we see that $L \cap V$ lies outside
$\Sigma'$. The same goes when $L$ is a
$\cal P$ lines.  So, again, the
intersection point is irrelevant.
\endproof

Now we take care of the strong case.
\begin{lemma}
In the strong case, every
special index is harmless.
\end{lemma}

\startproof
We want to see that
Lemma \ref{nuisance} holds in
the strong case.  The proof in the strong
case is exactly the same up until we get
to the last case, when
$M_i=\omega-2$ and the line $V$ of
capacity $\omega-1$ is the line
$x=\tau/2$.   There are $3$ cases to 
consider.
\newline
\newline
{\bf Case 1:\/}
Suppose that $\tau'<\omega'/3$.
Then $\Sigma'$ has width $\tau'$ and
$$\tau=\omega'-\tau'>2\tau'.$$
Hence the line of capacity $\omega-1$ lies outside
$\Sigma'$.  
\newline
\newline
{\bf Case 2:\/}
Suppose that $\tau'>\omega'/3$.
Then the width of $\Sigma'$ is $\omega'-2\tau'$,
the condition $\tau'>\omega'/3$ is
equivalent to the condition that
$\tau>2(\omega'-2\tau')$.  So, again
the line $x=\tau/2$ lies outside $\Sigma'$
\newline
\newline
{\bf Case 3:\/}
Suppose that $\tau'=\omega'/3$.
In this case $p'/q'=1/2$.
We are in the strong case, so
$\lambda=\omega'/\omega>1/3$.
Hence $\omega \leq 7$.  The only
possibility is $p/q=2/5$, and
we check this case by hand.
\endproof

\newpage


